Distributed Hierarchical Control for State Estimation With Robotic Sensor Networks

This paper addresses active state estimation with a team of robotic sensors. The states to be estimated are represented by spatially distributed, uncorrelated, stationary vectors. Given a prior belief on the geographic locations of the states, we cluster the states in moderately sized groups and propose a new hierarchical Dynamic Programming (DP) framework to compute optimal sensing policies for each cluster that mitigates the computational cost of planning optimal policies in the combined belief space. Then, we develop a decentralized assignment algorithm that dynamically allocates clusters to robots based on the pre-computed optimal policies at each cluster. The integrated distributed state estimation framework is optimal at the cluster level but also scales very well to large numbers of states and robot sensors. We demonstrate efficiency of the proposed method in both simulations and real-world experiments using stereoscopic vision sensors.

==> tcns-text/ack.tex <==
The authors would like to thank Prof. Ronald Parr from Duke University for valuable discussions on DP and MDP models and Prof. Philippos Mordohai from Stevens Institute of Technology for his insights on noise modeling and filtering in active sensing.

==> tcns-text/contribution.tex <==
Our controller is able to scale up to hundreds of hidden vectors and large decentralized teams of mobile robots.
This is diff

Different from point-based planners [8], [22], [23], [23]?[29], [19], [21], that degrade as the planning horizon grows, we do not sacrifice the quality of the sensor trajectories to gain the scalability.
The reason for this new capability is that the hierarchical structure essentially breaks the problem into three manageable parts.
First, it vertically integrates groups of local DPs into cluster DPs, which can then be horizontally integrated during the online multi robot control synthesis phase.



==> tcns-text/discuss.tex <==

%In this section we remark on the complexity of our algorithm.
%
%
%
%First, note that we solve a deterministic optimal control problem offline, i.e., before the real system starts operating.
%This requires us to assume that $\mbE[\bby_{i,k}] = \hbbx_{i,0} \; \forall i$ and $\forall k \in \mbN$, that is, future observations $\bby_{i,k}$ are expected to confirm our unbiased \emph{a priori} belief $\hbbx_{i,0}$.
%%, and we do not include deviations from that expectation in the objective function.
%Adaptive techniques that recompute based on observations acquired during the mission exist \cite{hollinger13}, and our method can be used in an adaptive scheme by solving the optimal control problem whenever $\normal{\hbbx_{i,k},\bbSigma_{i,k}}$ changes by some threshold.
%The KL divergence has been successfully applied in receding horizon controllers for this purpose \cite{Adurthi13}.
%
Our approach avoids having to represent combinations of 

does not incorporate the target uncertainty, modeled by the error covariance matrix, in the state-space. 
In these approaches, the state-space is a decision tree that captures all possible robot paths starting at $\bbp_0.$ 
Therefore, although individual states have lower dimension, the size of the state-space can grow exponentially large even for moderate planning horizons. 
Instead, the number of states in our hierarchical approach of the local and cluster DPs is constant in the planning horizon and depends primarily on the number of targets per cluster.
One could directly apply the method developed in Section~\ref{sec:st} to the multi target state-space
\begin{equation}\label{eq:brute}
\pair{ \cup_{i =1}^M \ccalW_i} \times \ccalC_1 \times \cdots \times \ccalC_M,
\end{equation}
which has a constant, user-specified number of states $N_\bbp \left( N_{\ccalL}N_{\ccalA} N_{\ccalT} +1 \right)^M$.
Unfortunately, any practical representation of $\Sym(2,\reals)_+$ leads to a large number for $N_{\ccalL}N_{\ccalA} N_{\ccalT} $.
Therefore, planning transitions over all states in \eqref{eq:brute} would be intractable.
Function approximation \cite{Bertsekas1996neuro} is a possibility, but the choices of approximating functions is not obvious.
Our hierarchical approach has $\abs{\ccalS_i} = N_\bbp \left( N_{\ccalL}N_{\ccalA} N_{\ccalT} +1 \right)$ states in the local state-space and $\abs{\ccalS} = 2^{\abs{\ccalT_p}}\abs{\ccalT_p} \left( \max_{i \in \set{1, \dots ,\abs{\ccalT_p}}} \abs{\ccalE_i} \right)\left( \max_{i \in \set{1, \dots ,\abs{\ccalT_p}}} K_i \right)$ in the $p$-th cluster's state-space, which is typically smaller than either the path-space approach for moderate planning horizons or the brute force method applied to the state-space \eqref{eq:brute} for a practical number of targets. 
%
The complexity of Algorithm~\ref{alg:VI} is $O(\abs{\ccalS_i}\abs{\ccalU_i})$ for the $i$-he local DP and, similarly, $O(\abs{\ccalT_p}\abs{\ccalU})$ for the $p$-th cluster DP.
%We note that we can accommodate actuation error in these algorithms without adding to the complexity, provided that we know the probability of outcome $\bbu'$ given control signal $\bbmu(\bbs)$, i.e., $P(\bbu'|\bbmu(\bbs)=\bbu)$, and that this probably is the same for any state.
%In this case, the deterministic DP becomes a Markov Decision Process (MDP), and the $Q$-function would need to account for all possible outcomes for each state-action pair, i.e.,
%\begin{equation}\label{eq:mdp}
%Q(\bbs,\bbu) = \sum_{\bbu' \in \ccalU} P(\bbu'|\bbmu(\bbs)=\bbu)\left(R(\bbs,\bbu') +  \gamma V(\bbPhi(\bbs,\bbu'))\right).
%\end{equation}



